Classical Klein-Gordon solutions, symplectic structures and isometry actions on AdS spacetimes

We study classical, real Klein-Gordon theory on Lorentzian Anti de Sitter (AdS_{1,d}) spacetimes with spatial dimension d. We give a complete list of well defined and bounded Klein-Gordon solutions for three types of regions on AdS: slice (time interval times all of space), rod hypercylinder (all of time times solid ball in space), and tube hypercylinder (all of time times solid shell in space). Hypercylinder regions are of natural interest for AdS since the neighborhood of the AdS-boundary is a tube. For the solution spaces of our regions we find the actions induced by the AdS isometry group SO(2,d). For all three regions we find one-to-one correspondences between initial data and solutions on the regions. For rod and tube regions this initial data can also be given on the AdS boundary. We calculate symplectic structures associated to the solution spaces, and show their invariance under the isometry actions. We compare our results to the corresponding expressions for (3+1)-dimensional Minkowski spacetime, arising from AdS_{1,3} in the limit of large curvature radius.

==> zzzzz_head_packs_hyphs.tex <==

\newcommand{\repa}{\RequirePackage}

\makeatletter\@ifpackageloaded{fixltx2e}{}{\repa{fixltx2e}}\makeatother
% provides some fixes to LaTeX2e, and the \TextOrMath command

\makeatletter\@ifpackageloaded{savesym}{}{\repa{savesym}}\makeatother
% There are a number of symbols that are defined by multiple packages.
% \savesymbol{XXX} renames a symbol from \XXX to \origXXX
% \restoresymbols{yyy}{XXX} renames \origXXX back to \XXX,
% and renames the current version of \XXX as \yyyXXX,
% see below at package stmaryrd for examples

\makeatletter\@ifpackageloaded{ae}{}{\repa{ae}}\makeatother
\makeatletter\@ifpackageloaded{aeguill}{}{\repa{aeguill}}\makeatother

\makeatletter\@ifpackageloaded{amsfonts}{}{\repa{amsfonts}}\makeatother
\makeatletter
\@ifpackageloaded{amsmath}{\PassOptionsToPackage{intlimits}{amsmath}}
	{\repa[intlimits]{amsmath}}\makeatother
\makeatletter\@ifpackageloaded{amssymb}{}{\repa{amssymb}}\makeatother
\makeatletter\@ifpackageloaded{amsxtra}{}{\repa{amsxtra}}\makeatother

\makeatletter\@ifpackageloaded{array}{}{\repa{array}}\makeatother
\makeatletter\@ifpackageloaded{babel}{}{\repa[english]{babel}}\makeatother
\makeatletter\@ifpackageloaded{bbm}{}{\repa{bbm}}\makeatother
%\makeatletter\@ifpackageloaded{bibspacing}{}{\repa{bibspacing}}\makeatother
% sets space between bibliography items to zero

\makeatletter\@ifpackageloaded{calc}{}{\repa{calc}}\makeatother
\makeatletter\@ifpackageloaded{cancel}{}{\repa{cancel}}\makeatother
%\repa {color} % replaced by xcolor
\makeatletter\@ifpackageloaded{colordvi}{}{\repa{colordvi}}\makeatother
\makeatletter\@ifpackageloaded{colortbl}{}{\repa{colortbl}}\makeatother

\makeatletter\@ifpackageloaded{dsfont}{}{\repa{dsfont}}\makeatother
\makeatletter\@ifpackageloaded{empheq}{}{\repa{empheq}}\makeatother
\makeatletter\@ifpackageloaded{esint}{}{\repa{esint}}\makeatother
\makeatletter\@ifpackageloaded{eurosym}{}{\repa{eurosym}}\makeatother

\makeatletter\@ifpackageloaded{fancybox}{}{\repa{fancybox}}\makeatother
\makeatletter\@ifpackageloaded{fancyhdr}{}{\repa{fancyhdr}}\makeatother
\makeatletter\@ifpackageloaded{float}{}{\repa{float}}\makeatother
\makeatletter\@ifpackageloaded{floatflt}{}{\repa{floatflt}}\makeatother
\makeatletter\@ifpackageloaded{fontenc}{}{\repa[OT2,T1]{fontenc}}\makeatother
%\makeatletter\@ifpackageloaded{graphicx}{}{\repa{graphicx}}\makeatother

\makeatletter\@ifpackageloaded{hhline}{}{\repa{hhline}}\makeatother
\makeatletter\@ifpackageloaded{ifthen}{}{\repa{ifthen}}\makeatother
% contains \ifthenelse{test}{if-code}{else-code}

%\repa {indentfirst}
%\makeatletter\@ifpackageloaded{inputenc}{}{\repa[latin1]{inputenc}}\makeatother
\makeatletter\@ifpackageloaded{inputenc}{}{\repa[UTF8]{inputenc}}\makeatother

\makeatletter\@ifpackageloaded{lamsarrow}{}{\repa{lamsarrow}}\makeatother
\makeatletter\@ifpackageloaded{latexsym}{}{\repa{latexsym}}\makeatother
\makeatletter
\@ifpackageloaded{letterspace}{}{\repa[letterspace=10]{letterspace}}
\makeatother
% \textls[#1]{#2} prints text #2 with letterspacing #1 times 1/1000em
% \lsstyle changes letterspacing to letterspace=10 within group

\makeatletter\@ifpackageloaded{longtable}{}{\repa{longtable}\setlongtables}\makeatother 
% if problems with longtables occur, delete .aux file,
% or run twice without \setlongtables

\makeatletter\@ifpackageloaded{makeidx}{}{\repa{makeidx}\makeindex}\makeatother
%\usepackage{mathabx} 		% not used, because produces ugly \leq and \geq
%\makeatletter\@ifpackageloaded{mathbbol}{}{\repa{mathbbol}}\makeatother
\makeatletter\@ifpackageloaded{mathrsfs}{}{\repa{mathrsfs}}\makeatother
\makeatletter\@ifpackageloaded{mathtools}{}{\repa{mathtools}}\makeatother

% microtype only for final runs, takes much compiling time ...
%\makeatletter\@ifpackageloaded{microtype}{}{\repa{microtype}}\makeatother

%\repa {minitoc}
% called in zzzzz_book because not wanted in articles

%\repa {multicol}	
% clashes with REVTEX, loaded separately in zzzzz_poster.tex

\makeatletter
\@ifpackageloaded{pb-diagram}{}{\repa{pb-diagram}}\makeatother
\makeatletter\@ifpackageloaded{pb-lams}{}{\repa{pb-lams}}\makeatother

\makeatletter\@ifpackageloaded{protosem}{}{\repa{protosem}}\makeatother

\usepackage{pdftricks}
\begin{psinputs}
	\usepackage{pstricks}
\end{psinputs}

\makeatletter\@ifpackageloaded{slashed}{}{\repa{slashed}}\makeatother

\savesymbol{bigtriangleup}% save the original Latex 2e version
\savesymbol{bigtriangledown} % of \bigtriangleup as \origbigtriangleup
\makeatletter\@ifpackageloaded{stmaryrd}{}{\repa{stmaryrd}}\makeatother
\restoresymbol{stmaryrd}{bigtriangleup}
\restoresymbol{stmaryrd}{bigtriangleup}
% restore original version of \bigtriangleup,
% save the St. Mary Road version as \stmaryroadbigtriangleup

\makeatletter\@ifpackageloaded{subfigure}{}{\repa{subfigure}}\makeatother

%\makeatletter\@ifpackageloaded{t1enc}{}{\repa{t1enc}}\makeatother
\makeatletter\@ifpackageloaded{theorem}{}{\repa{theorem}}\makeatother
%\makeatletter\@ifpackageloaded{tipa}{}{\repa{tipa}}\makeatother

\makeatletter\@ifpackageloaded{ulem}{}{\repa{ulem}\normalem}\makeatother % \uwave, \dashuline, \dotuline \sout, \xout
\makeatletter\@ifpackageloaded{undertilde}{}{\repa{undertilde}}\makeatother
\makeatletter\@ifpackageloaded{upgreek}{}{\repa{upgreek}}\makeatother
% upright greek letters, e.g.: \uplambda, \Uplambda
% use: e.g. upright \phi for fields, normal (italic) \phi for angles

\makeatletter\@ifpackageloaded{verbatim}{}{\repa{verbatim}}\makeatother

\makeatletter\@ifpackageloaded{wasysym}{}{\repa{wasysym}}\makeatother
\makeatletter\@ifpackageloaded{wrapfig}{}{\repa{wrapfig}}\makeatother

\makeatletter\@ifpackageloaded{xcolor}{}{\repa{xcolor}}\makeatother
\makeatletter\@ifpackageloaded{xspace}{}{\repa{xspace}}\makeatother
% \xspace command

\makeatletter\@ifpackageloaded{yhmath}{}{\repa{yhmath}}\makeatother

\makeatletter\@ifpackageloaded{hyperref}{}{\repa{hyperref}}\makeatother

% ==================================================================
% HYPHENATIONS

\hyphenation{Min-kows-ki Schr\"o-din-ger}


